DreamDPO: Aligning Text-to-3D Generation with Human Preferences via Direct Preference Optimization

Text-to-3D generation automates 3D content creation from textual descriptions, which offers transformative potential across various fields. However, existing methods often struggle to align generated content with human preferences, limiting their applicability and flexibility. To address these limitations, in this paper, we propose DreamDPO, an optimization-based framework that integrates human preferences into the 3D generation process, through direct preference optimization. Practically, DreamDPO first constructs pairwise examples, then compare their alignment with human preferences using reward or large multimodal models, and lastly optimizes the 3D representation with a preference-driven loss function. By leveraging pairwise comparison to reflect preferences, DreamDPO reduces reliance on precise pointwise quality evaluations while enabling fine-grained controllability through preference-guided optimization. Experiments demonstrate that DreamDPO achieves competitive results, and provides higher-quality and more controllable 3D content compared to existing methods. The code and models will be open-sourced.

==> sec/6_statement.tex <==
\newpage
\section{Impact Statement}
This paper advances the field of Text-to-3D generation by introducing DreamDPO, an optimization-based framework that integrates human preferences into the 3D generation process. By aligning generated content more closely with human preferences, our approach enhances the quality, controllability, and applicability of 3D content creation across various domains, including gaming, virtual reality, design, and digital media.

From an ethical perspective, our work raises considerations related to bias in human preference data, potential misuse in deepfake or unauthorized content generation, and the environmental impact of computationally intensive optimization processes. To mitigate these risks, we promote transparency by open-sourcing our code and models, allowing the research community to further evaluate and refine our approach. Additionally, we encourage responsible use of preference-driven generation techniques to ensure ethical applications.
